Fixing Hardware Security Bugs with Large Language Models

Novel AI-based code-writing Large Language Models (LLMs) such as OpenAI's Codex have demonstrated capabilities in many coding-adjacent domains. In this work we consider how LLMs maybe leveraged to automatically repair security relevant bugs present in hardware designs. We focus on bug repair in code written in the Hardware Description Language Verilog. For this study we build a corpus of domain-representative hardware security bugs. We then design and implement a framework to quantitatively evaluate the performance of any LLM tasked with fixing the specified bugs. The framework supports design space exploration of prompts (i.e., prompt engineering) and identifying the best parameters for the LLM. We show that an ensemble of LLMs can repair all ten of our benchmarks. This ensemble outperforms the state-of-the-art Cirfix hardware bug repair tool on its own suite of bugs. These results show that LLMs can repair hardware security bugs and the framework is an important step towards the ultimate goal of an automated end-to-end bug repair framework.

==> section/07Related.tex <==
\section{Related Prior Work\label{sec:related}}

Hardware bug repair has only recently been explored. The main distinction between hardware and software is that hardware has concurrent statements that can execute at the same instance of time whereas most software is sequential. 
The most relevant work is Cirfix \cite{ahmad_cirfix_2022}.  Cirfix attempts to localize bugs in RTL designs and then repair them. Cirfix provides the benchmarks that they develop for this purpose allowing us to apply our methods to compare results. 
While it is the closest work, there are fundamental differences in the approaches which limits direct comparisons. These differences are described in Table \ref{tbl:cirfix-comparison-table}. 
Cirfix performs both localization/identification of the bug and the repair. These two parts can be separated and a two-pronged approach combining a variety of approaches can be helpful. E.g. Tarsel \cite{wu_fault_2022} uses hardware-specific timing information and the program spectrum and captures the changes of executed statements to locate faults. Tarsel outperforms Cirfix on Cirfix's benchmarks as a fault localizer.
%Our repair approach has the advantage that an oracle is not needed. 
While Cirfix instruments an oracle to use the correct outputs to guide repairs, an oracle is not needed in our approach. % has the advantage that an oracle is not needed.
LLMs rely on the many examples of RTL code they have memorized to produce a correct version of the buggy code.

% Comparison to Cirfix
\begin{table}[h]
\caption{Comparison on Cirfix's benchmarks}
\label{tbl:cirfix-comparison-table}
\begin{tabular}{ll}
\hline
\textbf{Cirfix}         & \textbf{LLMs} \\ \hline \hline
Localization and repair & Repair only (assumes location) \\ \hline
Oracle-guided           & No oracle needed \\ \hline
\begin{tabular}[c]{@{}l@{}}Uses repair templates\\ and operators\end{tabular}   & Uses instructions \\ \hline
Iterative process        & One shot \\ \hline
\end{tabular}
\end{table}

The comparison of our work with Cirfix is shown in Table \ref{tbl:cirfix-comparison-results}. We use the best performing LLM i.e. code-davinci-002 at t=0.1 and generate one repair each for variations a and b. This is done to closely mirror the use case of Cirfix. By comparing the first example produced by the LLM, we evaluate only one attempt at repair. This attempt is then manually evaluated for correctness. We use variation a for the primary comparison as this variation uses no instructions to assist repairs. This variation produces 17.5 correct repairs as compared to Cirfix's 16. The half repair corresponds to fixing one numeric error out of 2 for the first benchmark. To further elicit the power of LLMs, we use variation b which includes a description of the type of bug to assist repair. We use the brief descriptions of bugs provided in Cirfix's github repository for this purpose. Variation b fixes 20 of the 32 benchmarks and collectively, LLMs (both variations) are able to repair 23.5 of the bugs.

% \begin{itemize}
%     \item Cirfix assumes unknown location
%     \item Cirfix has no instructions to assist
%     \item Cirfix has oracle guided repair
%     \item Cirfix is iterative, LLMs are one-shot
%     \item Cirfix targets functional bugs
%     \item Cirfix needs repair templates and operators
%     \item Cirfix provides one solution and says whether its correct or not through manual evaluation
%     \item time, caveat- cirfix could be faster on HPCs
% \end{itemize}


\begin{table}[]
\caption{Comparison on Cirfix's benchmarks}
\label{tbl:cirfix-comparison-results}
\resizebox{\linewidth}{!}{
\begin{tabular}{llcc}
\hline
\textbf{Project}                                                & \textbf{Defect Description}                                                                                                      & \textbf{Cirfix}           & \textbf{\begin{tabular}[c]{@{}c@{}}LLM\\ var a | b\end{tabular}} \\ \hline
decoder                                                         & Two numeric errors                                                                                                               & y                         & 1/2 | 1/2                                                        \\
(3 to 8)                                                        & \cellcolor[HTML]{C0C0C0}Incorrect assignment                                                                                     & \cellcolor[HTML]{C0C0C0}- & \cellcolor[HTML]{C0C0C0}- | -                                    \\ \hline
first\_counter                                                  & Incorrect sensitivity list                                                                                                       & y                         & y | y                                                            \\
overflow                                                        & \cellcolor[HTML]{C0C0C0}Incorrect increment of counter                                                                           & \cellcolor[HTML]{C0C0C0}y & \cellcolor[HTML]{C0C0C0}- | y                                    \\
                                                                & Incorrect reset                                                                                                                  & y                         & y | y                                                            \\ \hline
flip\_flop                                                      & Incorrect conditional                                                                                                            & y                         & - | -                                                            \\
                                                                & \cellcolor[HTML]{C0C0C0}if-statement branches swapped                                                                            & \cellcolor[HTML]{C0C0C0}y & \cellcolor[HTML]{C0C0C0}| y                                      \\ \hline
fsm\_full                                                       & Incorrect case statement                                                                                                         & -                         & - | -                                                            \\
                                                                & \cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}l@{}}Assignment to next state and\\ default in case statement omitted\end{tabular} & \cellcolor[HTML]{C0C0C0}y & \cellcolor[HTML]{C0C0C0}y | y                                    \\
                                                                & State omitted from senslist                                                                                                      & -                         & - | y                                                            \\
                                                                & \cellcolor[HTML]{C0C0C0}Incorrect blocking assignments                                                                           & \cellcolor[HTML]{C0C0C0}- & \cellcolor[HTML]{C0C0C0}- | -                                    \\ \hline
lshift\_reg                                                     & Incorrect blocking assignments                                                                                                   & y                         & - | y                                                            \\
                                                                & \cellcolor[HTML]{C0C0C0}Incorrect conditional                                                                                    & \cellcolor[HTML]{C0C0C0}y & \cellcolor[HTML]{C0C0C0}- | y                                    \\
                                                                & Incorrect sensitivity list                                                                                                       & y                         & y | y                                                            \\ \hline
mux\_4\_1                                                       & Three numeric errors                                                                                                             & -                         & y | y                                                            \\
                                                                & \cellcolor[HTML]{C0C0C0}Hex instead of binary numbers                                                                            & \cellcolor[HTML]{C0C0C0}- & \cellcolor[HTML]{C0C0C0}y | y                                    \\
                                                                & 1 bit instead of 4 bit output                                                                                                    & -                         & y | y                                                            \\ \hline
i2c                                                             & Incorrect sensitivity list                                                                                                       & y                         & - | -                                                            \\
                                                                & \cellcolor[HTML]{C0C0C0}Incorrect address assignment                                                                             & \cellcolor[HTML]{C0C0C0}- & \cellcolor[HTML]{C0C0C0}y | -                                    \\
                                                                & No command acknowledgement                                                                                                       & y                         & y | y                                                            \\ \hline
sha3                                                            & Off-by-one error in loop                                                                                                         & y                         & y | -                                                            \\
                                                                & \cellcolor[HTML]{C0C0C0}Incorrect assignment to wire                                                                             & \cellcolor[HTML]{C0C0C0}- & \cellcolor[HTML]{C0C0C0}y | -                                    \\
                                                                & Skipped buffer overflow check                                                                                                    & y                         & - | -                                                            \\
                                                                & \cellcolor[HTML]{C0C0C0}Incorrect bitwise negation                                                                               & \cellcolor[HTML]{C0C0C0}- & \cellcolor[HTML]{C0C0C0}y | y                                    \\ \hline
tate\_pairing                                                   & Incorrect logic for bitshifting                                                                                                  & -                         & - | -                                                            \\
                                                                & \cellcolor[HTML]{C0C0C0}Incorrect instantiation of modules                                                                       & \cellcolor[HTML]{C0C0C0}- & \cellcolor[HTML]{C0C0C0}y | y                                    \\
                                                                & Incorrect operator for bitshifting                                                                                               & -                         & y | y                                                            \\ \hline
\begin{tabular}[c]{@{}l@{}}reed\_solomon\\ decoder\end{tabular} & \begin{tabular}[c]{@{}l@{}}Insufficient register size\\ for decimal values\end{tabular}                                          & -                         & - | -                                                            \\
                                                                & \cellcolor[HTML]{C0C0C0}Incorrect sensitivity list for reset                                                                     & \cellcolor[HTML]{C0C0C0}y & \cellcolor[HTML]{C0C0C0}y | y                                    \\ \hline
\begin{tabular}[c]{@{}l@{}}sdram\\ controller\end{tabular}      & \begin{tabular}[c]{@{}l@{}}Incorrect assignments to registers\\ during synchronous reset\end{tabular}                            & y                         & y | 1/2                                                          \\
                                                                & \cellcolor[HTML]{C0C0C0}Numeric error in definitions                                                                             & \cellcolor[HTML]{C0C0C0}- & \cellcolor[HTML]{C0C0C0}y | y                                    \\
                                                                & Incorrect case statement                                                                                                         & -                         & - | y                                                            \\ \hline
                                                                & \multicolumn{1}{c}{}                                                                                                             & 16                        & 17.5 | 20                                                          \\ \cline{3-4} 
\end{tabular}
}
\end{table}


% How does Cirfix work?

% dataflow-based fault localization\\
% Instrumenting traditional hardware testbenches to guide repair\\
% CirFix
% uses genetic programming (GP), an iterative stochastic search technique, to find candidate repairs for defects in hardware designs.
% CirFix also makes use of readily-available artifacts in the hardware
% design process (e.g., testbenches, simulation environments) to diagnose and repair defects in a circuit description. We propose an
% approach to guide the search for a repair by instrumenting hardware testbenches to record the values of output wires at specified
% time intervals during a simulation of the circuit design. CirFix then
% performs a bit-level comparison of output wires against information
% for expected behavior to assess functional correctness of candidate
% repairs. CirFix employs a fixed point analysis of assignments made
% to internal registers and output wires to implicate statements and
% reduce the search space, enabling our approach to scale to large
% circuit designs in industry

% Fault localization happens only once

% oracle guided repair, final evaluation of correct repair is manual

==> section/preamble/preamblelistingsconf.tex <==
\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\definecolor{mymauve}{rgb}{0.58,0,0.82}

\makeatletter
\let\old@lstKV@SwitchCases\lstKV@SwitchCases
\def\lstKV@SwitchCases#1#2#3{}
\makeatother
\usepackage{lstlinebgrd}
\makeatletter
\let\lstKV@SwitchCases\old@lstKV@SwitchCases

\lst@Key{numbers}{none}{%
    \def\lst@PlaceNumber{\lst@linebgrd}%
    \lstKV@SwitchCases{#1}%
    {none:\\%
     left:\def\lst@PlaceNumber{\llap{\normalfont
                \lst@numberstyle{\thelstnumber}\kern\lst@numbersep}\lst@linebgrd}\\%
     right:\def\lst@PlaceNumber{\rlap{\normalfont
                \kern\linewidth \kern\lst@numbersep
                \lst@numberstyle{\thelstnumber}}\lst@linebgrd}%
    }{\PackageError{Listings}{Numbers #1 unknown}\@ehc}}
\makeatother

\usepackage{lstlinebgrd} % see http://www.ctan.org/pkg/lstaddons

\lstset{ 
%   escapeinside={(*@}{@*)},
%   backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}; should come as last argument
  basicstyle=\scriptsize,        % the size of the fonts that are used for the code
%   breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
%   captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
%   deletekeywords={...},            % if you want to delete keywords from the given language
%   escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
%   extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  frame=single,	                   % adds a frame around the code
%   keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  language=C,                 % the language of the code
%   morekeywords={*,...},            % if you want to add more keywords to the set
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\tiny\color{mygray}, % the style that is used for the line-numbers
%   rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
%   showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
%   showstringspaces=false,          % underline spaces within strings only
%   showtabs=false,                  % show tabs within strings adding particular underscores
%   stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{mymauve},     % string literal style
%   tabsize=2,	                   % sets default tabsize to 2 spaces
%   title=\lstname                   % show the filename of files included with \lstinputlisting; also try caption instead of title
%   %framesep=0pt,framerule=0pt,
%   %aboveskip=0pt,belowskip=0pt
}

